Banach-Mazur Parity Games and Almost-sure Winning Strategies

Two-player stochastic games are games with two 2 players and a randomised entity called "nature". A natural question to ask in this framework is the existence of strategies that ensure that an event happens with probability 1 (almost-sure strategies). In the case of Markov decision processes, when the event 2 of interest is given as a parity condition, we can replace the "nature" by two more players that play according to the rules of what is known as Banach-Mazur game [1]. In this paper we continue this research program by extending the above result to two-player stochastic parity games. As in the paper [1], the basic idea is that, under the correct hypothesis, we can replace the randomised player with two players playing a Banach-Mazur game. This requires a few technical observations, and a non trivial proof, that this paper sets out to do.

==> transfert.tex <==
\begin{theorem}[Transfert theorem]\label{thm:trsfrt}
  On a finite arena with parity objective, Eve wins almost-surely the
  stochastic game, if and only if Eve wins the two-player parity $\bm$
  game induced.
\end{theorem}

\begin{proof}
  Let $\calG$ be a parity stochastic game and $\bar{\calG}$ the
  two-player $\bm$ game induced. 

  Assume that $\e$ wins from $s$ in $\bar{\calG}$. By Theorem~\ref{thm:PosDet} there is a positional winning strategy of $\e$.
  
  Suppose, by contradiction that $\e$ does not win in the Stochastic game. By positional determinacy, there is a positional strategy $\tau$ that is positively winning for Adam. Let's play this strategy against all positional strategies of $\e$. For each of this combination of strategies, Adam wins positively the Markov chain, and thus, by Varacca Volzer, in the residual Banach Mazur game, Mazur wins. We have concluded that all the positional strategies of $\e$ are not winning, contradiction.







\DV{The other direction is exactly the same}
  Similalry, assume that $\e$ has an almost-sure
  winning strategy $\sigma$ from $s$ in $\calG$. 

Consider the set $X$ of memoryless strategies for $\e$ that win almost surely against all memoryless strategies for
  $\a$. Let $Y$ be the set of other memoryless strategies for $\e$, those who do not win almost surely against some memoryless strategy fo $\a$. They are not winning strategies. For each $\sigma\in Y$ choose one such $\tau_\sigma$.
  Clearly in the residual Banach Mazur game, Mazur has a winning strategy. So the strategies in $Y$ are not winning.

 Suppose all the strategies of $X$ are also not winning. By Theorem~\ref{thm:PosDet}, we know that no strategy is winning (as no positional one is), and thus there is a positional strategy $\tau$ that that make Eve and Adam lose. Let's play this strategy against all positional strategies of $X$. By Varacca Volzer, in the residual Markov Chain, Adam wins positively. We have concluded that the strategies of $X$ are also not winning almost surely. Thus no positional strategy is wnning almost surely, contradiction.


We will
  show that $\sigma$ is winning as well in $\bar{\calG}$ from $s$.
  
  By Theorem~\ref{thm:PosDet} we can assume that $\sigma$ is
  memoryless, toward a contradiction assume that $\sigma$ is losing in
  $\bar{\calG}$ from $s$. Formally, assume that $\a$ has a strategy
  $\tau$ in $\bar{\calG}(\sigma)$ such that against any strategy
  $\bsigma$ for $\b$, there exists a strategy $\mtau$ for $\m$ such
  that the induced play is not in $\parity$.  Since $\parity$ is a
  Borel set, the game played between $\b$ and $\m$ on the residual
  tree $\bar{\calG}(\sigma,\tau)$ is determined.  Therefore, there
  exists a strategy for $\m$ such that against any strategy for $\b$
  the induced play is in $\parity$. Moreover, $\tau$ can be chosen
  memoryless~\cite{FOSSACS}. Since $\m$ has the lead and $\tau$ is
  memoryless the results in~\cite{VV} apply, it follows that $\tau$ is
  positively winning from $s$ in the MDP $\calG(\sigma)$, that is
  $\prob{s}^{\sigma,\tau}(\parity) < 1$ a contradiction, thus $\sigma$
  is winning in $\bar{\calG}$ from $s$.



\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mainGandalf.tex"
%%% End:

